Jointly Assigning Processes to Machines and Generating Plans for Autonomous Mobile Robots in a Smart Factory

A modern smart factory runs a manufacturing procedure using a collection of programmable machines. Typically, materials are ferried between these machines using a team of mobile robots. To embed a manufacturing procedure in a smart factory, a factory operator must a) assign its processes to the smart factory's machines and b) determine how agents should carry materials between machines. A good embedding maximizes the smart factory's throughput; the rate at which it outputs products. Existing smart factory management systems solve the aforementioned problems sequentially, limiting the throughput that they can achieve. In this paper we introduce ACES, the Anytime Cyclic Embedding Solver, the first solver which jointly optimizes the assignment of processes to machines and the assignment of paths to agents. We evaluate ACES and show that it can scale to real industrial scenarios.

==> old_text.tex <==
 Before we can present our formulation, however, we need to introduce some notation.

\para{Notation.} Let $\zIn{\m{i}}$ be the set of tokens consumed by a process that machine $\m{i}$ can run, that is:

\vspace{-3mm}
\begin{equation*}
    \zIn{\m{i}} := \bigcup_{\p{j} \in \mProc{\m{i}}} \{\tk{k} \in \allTk{} : \outTkType{\p{j}}{k} > 0\}.
\end{equation*}
\vspace{-2mm}

Regardless of the process assigned to machine $\m{i}$, it will only ever consume tokens in $\zIn{\m{i}}$. Conversely, let $\consume{\tk{i}}$ be the set of machines which can run a process that consumes token $\tk{i}$, that is, $\consume{\tk{i}} := \{\m{j} \in \allM{} : \tk{i} \in \zIn{\m{i}}\}$. Regardless of how a smart factory is configured, token $\tk{i}$ will only be consumed by machines in $\consume{\tk{i}}$. Similarly, let $\zOut{\m{i}}$ be the set of tokens emitted by a process that machine $\m{i}$ could run, and $\emit{\tk{i}}$ be the set of machines which can run a process that emits token $\tk{i}$.




If an agent ends a timestep on a machine's input cell, it can deposit its token in the machine's input buffer. If an agent which isn't carrying a token ends a timestep on a machine's output cell, it can pick up a token from the machine's output buffer. An agent may not pick up or deposit tokens under any other circumstances. The token that agent $\ag{i}$ is carrying on timestep $t$ is denoted $\agTk{\ag{i}}{t}$. If agent $\ag{i}$ is not carrying a token on timestep $t$, $\agTk{\ag{i}}{t}$ has the special value $\nullTk{}$, where $\nullTk{}$ is the null token. The state $(\agCl{\ag{i}}{t}, \agTk{\ag{i}}{t})$ of agent $\ag{i}$ at timestep $t$ is its location and the token it is carrying.

\para{Wait Time Vector.} Some machines may be able to run their processes faster than others. We can slow down a machine, synchronizing it with the rest of the factory, by instructing it to wait for a short amount of time whenever it finishes running its process. We represent these instructions with a length $|M|$ vector called the wait time vector $\wVec{}$. The field $\wVecF{i}$ contains the number of timesteps that machine $\m{i}$ should wait after finishing its process.

\para{Movement Tensor.} Knowing the location of every token at every timestep does not tell you how the tokens move. Since copies of the same token are indistinguishable, there may be multiple ways to move tokens to produce a configuration seen at timestep $t + 1$ from a configuration seen at timestep $t$. We eliminate this ambguity with the movement tensor $\mvT{}$, a $|\layoutE{}| \times (\ct{} + 1) \times |\allTkWithNull{}|$ tensor. The field $\mv{\cl{i}}{\cl{j}}{t}{\tk{k}} \in \{0, 1\}$ indicates iff a copy of token $\tk{k}$ moves from $\cl{i}$ to $\cl{j}$ on timestep $t$. 

The FLAT SFEP is easier to solve as a MILP than the SFEP because it requires fewer constraints. The difficulty of a MILP grows exponentially with the number of constraints that it contains. Formulating the SFEP as a MILP introduces a binary variable indicating whether cell $\cl{i}$ contains agent $\ag{j}$ on timestep $t$ for every (cell, timestep, agent) combination. A SFEP instance may have dozens of agents. Solving it may involve considering embedding with dozens of timestep. As a result, there may be thousands of these variables and their associated constraints. Solving FLAT SFEP needs fewer of these variables since there are usually fewer tokens than agents and it has a limited number of timesteps.




\para{Buffer Entry and Exit Constraints.} These constraints specify how tokens can enter and exit buffers.

\para{Constraint 5.} Over the course of a transport plan, the number of copies of token $\tk{j} \in \allTk{}$ that machine $\m{i}$ consumes and that
enter its input buffer must be the same.

\vspace{-4mm}
\begin{align*}
    % Introduction
    &\forall\ \m{i} \in \allM{},\ \forall\ \tk{j} \in \allTk{},\\%
    %L.H.S.
    &\sum_{t = 0}^\ct{} \en{\mIn{\m{i}}}{t}{\tk{j}}
    %R.H.S.
    = \sum_{\mathclap{\p{k} \in \allP{}}} \rate{\m{i}}{\p{j}} \cdot \inTkType{\p{k}}{j} \cdot \ct{}.%
\end{align*}
\vspace{-3mm}


\para{Constraint 6.} Over the course of a transport plan, the number of copies of token $\tk{j}$ that machine $\m{i}$ emits and that
exit its output buffer must be the same.

\vspace{-4mm}
\begin{align*}
    % Introduction
    &\forall\ \m{i} \in \allM{},\ \forall\ \tk{j} \in \allTk{},\\%
    %L.H.S.
    &\sum_{t = 0}^\ct{} \ex{\mOut{\m{i}}}{t}{\tk{j}}
    %R.H.S.
    = \sum_{\mathclap{\p{k} \in \allP{}}} \rate{\m{i}}{\p{j}} \cdot \outTkType{\p{k}}{j} \cdot \ct{}.%
\end{align*}
\vspace{-3mm}

\para{Token Movement Constraints.} These constraints specify how tokens move through the factory.

\para{Constraint 7.} Each timestep $t$, a token $\tk{j} \in \allTkWithNull{}$ on cell $\cl{i}$ must wait on cell $\cl{i}$, move to an adjacent cell, or enter an input buffer. Recall that each vertex in the movement graph has a self-loop, and that the field $\mv{\cl{i}}{\cl{i}}{t}{\tk{j}}$ indicates if token $\tk{j}$ waits at cell $\cl{i}$ on timestep $t$.

\vspace{-4mm}
\begin{align*}
\forall\ \cl{i}, t&, \tk{j} \in C \times [0..\ct{}] \times \allTkWithNull{},\ \at{\cl{i}}{t}{\tk{j}} = \\
&\sum_{\mathclap{\cl{k} \in \adj{\cl{i}}}} \mv{\cl{i}}{\cl{k}}{t}{\tk{j}} + 
\begin{cases}
\en{\cl{i}}{t}{\tk{j}} &\cl{i} \in \allCIn{}\\
0               &\text{otherwise}
\end{cases}.
\end{align*}
\vspace{-2mm}

\para{Constraint 8.} If token $\tk{k}$ is not the null token, that is, $\tk{k} \in \allTk{}$, the number of copies of token $\tk{k}$ on cell $\cl{i}$ at timestep $t+1$ is equal to the number of copies of token $\tk{k}$ that move to, wait at, or exit an output buffer onto cell $\cl{i}$ at timestep $t$. Let $\allCOut{}$ be the set of all output cells. 

\vspace{-4mm}
\begin{align*}
\forall\ \cl{i}, t&, \tk{j} \in C \times [0..\ct{}] \times \allTk{},\ \at{\cl{i}}{t + 1}{\tk{j}} = \\
&\sum_{\mathclap{\cl{k} \in \adj{\cl{i}}}} \mv{\cl{k}}{\cl{i}}{t}{\tk{j}} + 
\begin{cases}
\ex{\cl{i}}{t}{\tk{j}} &\cl{i} \in \allCOut{}\\
0               &\text{otherwise}
\end{cases}.
\end{align*}
\vspace{-2mm}

\para{Constraint 9.} The number of copies of the null token $\tk{0}$ on cell $\cl{i}$ at timestep $t+1$ is equal to the number of copies of the null token $\tk{0}$ that move to, wait at, or replace a non-null token entering an input buffer on cell $\cl{i}$ at timestep $t$.

\vspace{-4mm}
\begin{align*}
\forall\ \cl{i}, t& \in C \times [0..\ct{}],\ \at{\cl{i}}{t + 1}{\tk{0}} = \\
&\sum_{\mathclap{\cl{k} \in \adj{\cl{i}}}} \mv{\cl{k}}{\cl{i}}{t}{\tk{j}} + 
\begin{cases}
\ex{\cl{i}}{t}{\tk{j}} &\cl{i} \in \allCOut{}\\
0               &\text{otherwise}
\end{cases}
-
\begin{cases}
\ex{\cl{i}}{t}{\tk{j}} &\cl{i} \in \allCOut{}\\
0               &\text{otherwise}
\end{cases}.
\end{align*}
\vspace{-2mm}

In the Multi Agent Pickup and Delivery (MAPD) problem~\cite{MAPD}, for example, a team of robots is tasked with transporting items found in a warehouse to packaging stations. To solve this problem, each transportation task has to be assigned to an agent and then each agent assigned a path which completes its tasks. The MAPD problem has been solved optimally using conflict-based search~\cite{ECBS_TA}. Other approaches such as~\cite{CCPP} sacrifice optimality for scalability.

The Collective Construction (CC) problem is related to the SFEP and also involves MAPF. In this problem, 



\begin{algorithm}[t]
\small
\caption{\convertToSFEP{}$(\assignM{}, \rateM{}, \bInM{}, \bOutM{}, \atT{}, \mvT{}, \enT{}, \exT{})$}
\label{alg:toSFEPEmb}
\begin{algorithmic}[1]
%
\STATE $\agClM{} \gets$ an empty $n \times (T+1)$ matrix
\COMMENT{Stores agent positions}
%
\STATE $\agTkM{} \gets$ an empty $n \times (T+1)$ matrix
\COMMENT{Stores agent cargo}
%
\STATE $i \gets 0$ 
\COMMENT{Agent index}
%
\FOR{$(\cl{j}, \tk{k}) \in \allCl{} \times \allTk{}$}
%
  \IF{$\at{\cl{j}}{0}{\tk{k}} = 1$}
  \label{ln:find_agent_starts}
  
    % Initialize Agent
    \STATE $\agCl{\ag{i}}{0} \gets \cl{j}$
    \STATE $\agTk{\ag{i}}{0} \gets \tk{k}$
    \label{ln:initialize_agents}
    
    
    % Compute Agent Plan
    \FOR{$t$ from $0$ to $\ct{}$}

      % Move Agent to Adjacent Cell
      % For all neighbors
      \FOR{$\cl{l} \in \adj{\agCl{\ag{i}}{t}}$}
      \label{ln:move_check}
        % If the agent moves to the neighbor
        \IF{$\mv{\agCl{\ag{i}}{t}}{\cl{l}}{t}{\agTk{\ag{i}}{t}} = 1$}
            % Set its state accordingly
            \STATE $\agCl{\ag{i}}{t + 1} \gets \cl{l}$
            \STATE $\agTk{\ag{i}}{t + 1} \gets \agTk{\ag{i}}{t}$
            \label{ln:move_action}
        \ENDIF
      \ENDFOR

      % If the token that the agent is following is removed
      \IF{$\remove{\agCl{\ag{i}}{t}}{t}{\agTk{\ag{i}}{t}}$}
        % Find the token that it is replaced by
        \FOR{$\tk{m} \in \allTk{}$}
          \IF{$\place{\agCl{\ag{i}}{t}}{t}{\tk{m}}$}
            % Set its state accordingly
            \STATE $\agCl{\ag{i}}{t + 1} \gets \agCl{\ag{i}}{t}$
            \STATE $\agTk{\ag{i}}{t + 1} \gets \tk{m}$
          \ENDIF
        \ENDFOR
      \ENDIF

      % If agent puts down token
      \IF{$\en{\agCl{\ag{i}}{t}}{t}{\agCl{\ag{i}}{t}} = 1$}
      \label{ln:deposit_check}
      % Set its state accordingly
        \STATE $\agCl{\ag{i}}{t + 1} \gets \agCl{\ag{i}}{t}$
        \STATE $\agTk{\ag{i}}{t + 1} \gets \tk{0}$
        \label{ln:deposit_action}
      \ENDIF

      % If agent picks up token
      \FOR{$\tk{m} \in \allTk{}$}
      \label{ln:pick_up_check}
        \IF{$\ex{\agCl{\ag{i}}{t}}{t}{\tk{m}}$}
          % Set its state accordingly
          \STATE $\agCl{\ag{i}}{t + 1} \gets \agCl{\ag{i}}{t}$
          \STATE $\agTk{\ag{i}}{t + 1} \gets \tk{m}$
          \label{ln:pick_up_action}
        \ENDIF
      \ENDFOR

      % Increment agent counter
      \STATE $i \gets i + 1$
      
    \ENDFOR % t from 0 to \ct{}
    
  \ENDIF % at(cj, 0, zk) = 0
\ENDFOR %(cj, zk) in C x Z

\RETURN $(\assignM{}, \rateM{}, \bInM{}, \bOutM{}, \agClM{}, \agTkM{})$
%
\end{algorithmic}
\end{algorithm}


\para{Buffer Entry and Exit Tensors.} Let $\allMIn{}$ and $\allMOut{}$ be the set of all input and output cells. Let $\mIn{\m{i}}$ and $\mOut{\m{i}}$ be machine $\m{i}$'s input and output cell (if they exist). The buffer entry and exit tensors $\placeT{}$ and $\removeT{}$ are $|\allMIn{}| \times (\ct{} + 1) \times |\allTk{}|$ and $|\allMOut{}| \times (\ct{} + 1) \times |\allTk{}|$ tensors.  The fields $\en{\mIn{\m{i}}}{t}{\tk{j}} \in \{0, 1\}$ and $\ex{\mOut{\m{i}}}{t}{\tk{j}} \in \{0, 1\}$ indicate if a copy of token $\tk{j}$ enters machine $\m{i}$'s input buffer and exits its output buffer on timestep $t$.

Tokens may not be placed on or removed from the factory floor for any other reason. 

 In a traditional smart factory, agents are autonomous mobile robots. In a mag-lev based smart factory, such as BOSCH's ctrlX Flow$^{\text{6D}}$~\cite{BOSCH_maglev}, agents are magnetically levitating shuttles. 

 To accomplish this, we need to turn our solution to the FLAT SFEP problem into an anytime algorithm. 
